FreeControl: Training-Free Spatial Control of Any Text-to-Image Diffusion Model with Any Condition

Recent approaches such as ControlNet offer users fine-grained spatial control over text-to-image (T2I) diffusion models. However, auxiliary modules have to be trained for each type of spatial condition, model architecture, and checkpoint, putting them at odds with the diverse intents and preferences a human designer would like to convey to the AI models during the content creation process. In this work, we present FreeControl, a training-free approach for controllable T2I generation that supports multiple conditions, architectures, and checkpoints simultaneously. FreeControl designs structure guidance to facilitate the structure alignment with a guidance image, and appearance guidance to enable the appearance sharing between images generated using the same seed. Extensive qualitative and quantitative experiments demonstrate the superior performance of FreeControl across a variety of pre-trained T2I models. In particular, FreeControl facilitates convenient training-free control over many different architectures and checkpoints, allows the challenging input conditions on which most of the existing training-free methods fail, and achieves competitive synthesis quality with training-based approaches.

==> table/cond2img_small.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{1.0\linewidth}{17mm}{
\begin{tabular}{lccc}
\toprule[1.5pt]


\multirow{2}{*}{Method} & \multicolumn{3}{c}{Depth}\\ \cmidrule(r){2-4}
               & Self-Sim~$\downarrow$ & CLIP~$\uparrow$  & LPIPS~$\uparrow$  \\ \midrule[0.5pt]
\color[HTML]{9b9b9b}ControlNet~\cite{zhang2023controlNet}     & \color[HTML]{9b9b9b}0.042    & \color[HTML]{9b9b9b}0.300 & \color[HTML]{9b9b9b}0.665 &  \color[HTML]{9b9b9b}0.040    & \color[HTML]{9b9b9b}0.291 & \color[HTML]{9b9b9b}0.609 & \color[HTML]{9b9b9b}0.070    & \color[HTML]{9b9b9b}0.314 & \color[HTML]{9b9b9b}0.668 &  \color[HTML]{9b9b9b}0.058    & \color[HTML]{9b9b9b}0.306 & \color[HTML]{9b9b9b}0.645 & \color[HTML]{9b9b9b}0.079    & \color[HTML]{9b9b9b}0.304 & \color[HTML]{9b9b9b}0.637 \\
\color[HTML]{9b9b9b}T2I-Adapter    & \color[HTML]{9b9b9b}0.052    & \color[HTML]{9b9b9b}0.290 & \color[HTML]{9b9b9b}0.689 & \color[HTML]{9b9b9b}-        & \color[HTML]{9b9b9b}-     & \color[HTML]{9b9b9b}-     & \color[HTML]{9b9b9b}0.096    & \color[HTML]{9b9b9b}0.290 & \color[HTML]{9b9b9b}0.648 \color[HTML]{9b9b9b}& \color[HTML]{9b9b9b}0.071    & \color[HTML]{9b9b9b}0.314 & \color[HTML]{9b9b9b}0.673 & \color[HTML]{9b9b9b}-        & \color[HTML]{9b9b9b}-     & \color[HTML]{9b9b9b}-      \\
\color[HTML]{9b9b9b}Uni-ControlNet & \color[HTML]{9b9b9b}0.044    & \color[HTML]{9b9b9b}0.295 & \color[HTML]{9b9b9b}0.539 & \color[HTML]{9b9b9b}0.050    & \color[HTML]{9b9b9b}0.301 & \color[HTML]{9b9b9b}0.553 & \color[HTML]{9b9b9b}0.050    & \color[HTML]{9b9b9b}0.301 & \color[HTML]{9b9b9b}0.553 & \color[HTML]{9b9b9b}0.061    & \color[HTML]{9b9b9b}0.303 & \color[HTML]{9b9b9b}0.636 & \color[HTML]{9b9b9b}-        &  \color[HTML]{9b9b9b}-    & \color[HTML]{9b9b9b}-   \\ %\hline 
\addlinespace
SDEdit-0.75~\cite{meng2021sdedit}    & 0.108    & 0.306 & 0.582 & 0.123    & 0.288 & 0.375 & 0.135    & 0.281 & 0.361 & 0.153    & 0.294 & 0.327 & 0.128    & 0.284 & 0.456 \\
SDEdit-0.85~\cite{meng2021sdedit}    & 0.139    & 0.319 & \textbf{0.670} & 0.153    & 0.305 & 0.485 & 0.139    & 0.300 & 0.485 & 0.165    & 0.304 & 0.384 & 0.147    & 0.298 & 0.512 \\
P2P~\cite{hertz2022prompt-to-prompt}            & 0.078    & 0.253 & 0.298 & 0.112    & 0.253 & 0.194 & 0.194    & 0.251 & 0.096 & 0.142    & 0.248 & 0.167 & 0.100    & 0.249 & 0.198 \\
PNP~\cite{tumanyan2023plug-and-play} & \textbf{0.074}    & 0.282 & 0.417 & 0.098    & 0.286 & 0.271 & 0.158    & 0.267 & 0.221 & 0.126    & 0.287 & 0.268 & 0.107    & 0.286 & 0.347  \\
\rowcolor{gray!10} Ours           & \textbf{0.074}    & \textbf{0.338} & 0.667 & \textbf{0.075}  &  \textbf{0.337} & \textbf{0.561} & \textbf{0.086}    & \textbf{0.337} & \textbf{0.593} & \textbf{0.077}    & \textbf{0.307} & \textbf{0.477} & \textbf{0.086}    & \textbf{0.335} & \textbf{0.629} \\ 
 \bottomrule[1.5pt]
\end{tabular}
}
\centering
\caption{\textbf{Quantitative results on controllable T2I diffusion.}
FreeControl consistently outperforms all training-free baselines in structure preservation, image-text alignment and appearance diversity as measured by Self-similarity distance, CLIP score and LPIPS distance. It achieves competitive structure and appearance scores with the training-based baselines while demonstrate stronger image-text alignment.
}\vspace{-1.5em}
\end{table*}
